Ultrafast coherent control of spinor Bose-Einstein condensates using stimulated Raman adiabatic passage

We propose the use of stimulated Raman adiabatic passage (STIRAP) to offer a fast high fidelity method of performing SU(2) rotations on spinor Bose Einstein condensates (BEC). Past demonstrations of BEC optical control suffer from difficulties arising from collective enhancement of spontaneous emission and inefficient two-photon transitions originating from selection rules. We present here a novel scheme which allows for arbitrary coherent rotations of two-component BECs while overcoming these issues. Numerical tests of the method show that for BECs of \ce{^{87}Rb} with up to $ 10^4 $ atoms and gate times of $ \SI{1}{\micro\second} $, decoherence due to spontaneous emission can be suppressed to negligible values.

==> fidelityplot.tex <==
%% Creator: Inkscape inkscape 0.48.4, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'fidelityplot.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{641.99907227bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.75078043)%
    \put(0.02,0){\includegraphics[width=\unitlength]{fidelityplotshit.pdf}}%
\small
    \put(0.02506246,0.06496303){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$10^{-10}$}}}%
    \put(0.03706246,0.20031871){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$10^{-8}$}}}%
    \put(0.03706246,0.33567601){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$10^{-6}$}}}%
    \put(0.03706246,0.47266227){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$10^{-4}$}}}%
    \put(0.03706246,0.60801957){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$10^{-2}$}}}%
    \put(0.03706246,0.74500617){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$10^{+0}$}}}%
    \put(0.09843754,0.02218617){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$1$}}}%
    \put(0.99000000,0.02218617){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$10$}}}%
    \put(0.02421869,0.30624847){\color[rgb]{0,0,0}\rotatebox{90}{\makebox(0,0)[lb]{\smash{$D(\rho,\sigma) = 1 - F(\rho,\sigma)$}}}}%
    \put(0.51406231,0.00937308){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$t_\textup{end}/\tau$}}}%
    \put(0.16155788,0.16582542){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$N=10^3, \Omega_0=10^3\Gamma$}}}%
    \put(0.22205835,0.28613557){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\textcolor{green}{\smash{$N=10^4, \Omega_0=10^3\Gamma$}}}}%
    \put(0.2705003,0.51638908){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\textcolor{magenta}{\smash{$N=10^5, \Omega_0=10^3\Gamma$}}}}%
    \put(0.62458915,0.53138288){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\textcolor{purple}{\smash{$N=10^6, \Omega_0=10^3\Gamma$}}}}%
    \put(0.2705003,0.40399707){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\textcolor{red}{\smash{$N=10^3, \Omega_0=10^2\Gamma$}}}}%
    \put(0.37458915,0.58731167){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\textcolor{orange}{\smash{$N=10^4, \Omega_0=10^2\Gamma$}}}}%
    \put(0.68752587,0.66874552){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\textcolor{blue}{\smash{$N=10^6, \Omega_0=10^2\Gamma$}}}}%
    \put(0.12752587,0.63874552){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\textcolor{violet}{\smash{$N=10^5, \Omega_0=10^2\Gamma$}}}}%
  \end{picture}%
\endgroup%

